Dense Human Body Correspondences Using Convolutional Networks

We propose a deep learning approach for finding dense correspondences between 3D scans of people. Our method requires only partial geometric information in the form of two depth maps or partial reconstructed surfaces, works for humans in arbitrary poses and wearing any clothing, does not require the two people to be scanned from similar viewpoints, and runs in real time. We use a deep convolutional neural network to train a feature descriptor on depth map pixels, but crucially, rather than training the network to solve the shape correspondence problem directly, we train it to solve a body region classification problem, modified to increase the smoothness of the learned descriptors near region boundaries. This approach ensures that nearby points on the human body are nearby in feature space, and vice versa, rendering the feature descriptor suitable for computing dense correspondences between the scans. We validate our method on real and synthetic data for both clothed and unclothed humans, and show that our correspondences are more robust than is possible with state-of-the-art unsupervised methods, and more accurate than those found using methods that require full watertight 3D geometry.

==> acknowledgement.tex <==
\section{Acknowledgement}
Hao's research team is supported in part by Adobe, Oculus \& Facebook, Sony, Pelican Imaging, Panasonic, Embodee, Huawei, the USC Integrated Media System Center, the Google Faculty Research Award, The Okawa Foundation Research Grant, the Office of Naval Research (ONR) / U.S. Navy, under award number N00014-15-1-2639, the Office of the Director of National Intelligence (ODNI), and Intelligence Advanced Research Projects Activity (IARPA), under contract number 2014-14071600010. Qixing has obtained gift awards from Adobe, Intel, and the National Science Foundation (NSF), under grant number DMS-1521583. Etienne is supported by NSF, under grant number DMS-1304211. The views and conclusions contained herein are those of the authors and should not be interpreted as necessarily representing the official policies or endorsements, either expressed or implied, of ODNI, IARPA, or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Governmental purpose notwithstanding any copyright annotation thereon.

==> approach.tex <==
\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\linewidth]{figures/segmentation/segmentation.pdf}
\end{center}
   \caption{Segmentation.}
\label{fig:segmentation}
\end{figure}

\section{Our Approach}

\subsection{Overlapping smooth}
\label{sec:smoothing}
\textcolor{red}{One contribution of this paper is that it learns a smooth descriptor without using triplet sampling, meaning that we can learn a network fast and doesn't need so many hardware.}

\cosimo{When we tried to train a classification model to detect which part of the body a certain pixel is in, traditional method tries to assign a label to each class, however if connections between different labels are not considered, non smoothness will be induced on the boundaries of regions as the network tries to separate two points, although similar in the actual setting, away as they are not on the same region.}

\cosimo{I think we can choose an example to show that by using overlapping segmentations it does help.}

==> correspondence.tex <==
% !TEX root = egpaper_for_review.tex
\section{Correspondence Computation}
Once we use our trained model to predict per-pixel feature descriptors for each depth image, we can use these descriptors to establish correspondences across depth images. This is done simply by a nearest neighbor search in the feature space. Since depth images only provide partial observations of the human body, the correspondence computation should consider the fact that the overlapping regions between two depth images is often smaller than the regions observed by each of the depth images alone. Thus, we need a strategy to discard unreliable correspondences coming from non-overlapping regions. We achieve this goal by enforcing spatial constraints among the correspondences since neighboring pixels in a source depth image are likely to be matched to neighboring pixels in the target depth image. More specifically, we build a connection graph in the source depth image where each pixel is denoted by a vertex. Two neighboring pixels $p^s_1$ and $p^s_2$ in the source depth image (we only consider horizontal or vertical neighbors) are connected by an edge if their corresponding pixels $p^t_1$ and $p^t_2$ in the target image represent 3D points with a Euclidean distance below a certain threshold ($10$ centimeters in our example). We then extract the largest connected component of this graph and discard the remaining correspondences.

We can further extend our method to establish correspondences directly between 3D models. We achieve this goal by first rendering depth maps of a 3D model from various multiple viewpoints and computing per-pixel descriptors for each of these depth images. A single 3D vertex might be then be visible in multiple images. In this case, we simple average the descriptors computed for this vertex from every depth image it is visible in to generate per-vertex descriptors in 3D.

==> data.tex <==
\section{Training Data}
\cosimo{what kind of data we used for training, how we process them (on mesh we do segmentation, on image we do normalization)}
\subsection{SCAPE dataset}
\cosimo{For the scape dataset we tried to segment it into 100 regions,
and we apply 10 different segmentations on it.
For every pose we use 144 cameras.}

\cosimo{Need to show that for every points within a certain range, there is a segmentation that contains them in the same region.}

\subsection{MIT dataset}
\cosimo{for every identity we segment it into 100 regions,
for 5 different segmentations.
And for every sequence we use 36 cameras}

\subsection{Yobi dataset}
\cosimo{we manually labeled 33 landmarks on each model
and use 144 cameras to synthesize depth images}

\subsection{Preprocessing}
\cosimo{Every depth image is of 512x512 pixels.
Character in the depth image has height around 250 to 260 pixels.
This is comparable to commercial depth cameras.
For example Kinect one has 512x424 resolution, where a human of height 1.7m standing 2.5 m away from camera has height around XXX pixels.  (Let's measure this number sometime.)}

\cosimo{For every depth image we assume the background can be clearly cut out.
This can be done by simply recording the background, and subtract it when recording.
Also we can discard pixels that are very far away.
For indoor setting this is enough to cut a clear foreground.}

Only the mesh of human is rendered onto the depth image, and the background is simply zero-filled. We do not try to simulate any fake background, as due to the limitation of depth camera by now it's not suitable for outdoor capturing, and for indoor capturing setting it is easy to cut out the background by applying motion detection and distance thresholding. ??? shows that such a naive implementation can easily cut out a clear foreground on depth images captured by Kinect.

For foreground pixels, we subtract the mean depth of all pixels within a frame from all foreground pixels, leading a zero-mean depth image. This process is frame independent and can be easily applied to newly recorded images. 
Note that we did not try to normalize each frame by dividing a standard derivation computed per frame, because it will induce inconsistency for people with different poses or different views.

However, it is worth mentioning that when using another depth camera with different unit of measurement on depth or different field of view, a constant scaling factor should be derived from the intrinsic matrix of camera, and be multiplied to every frame captured to maintain a range of depth to maintain the range of data consistent to the data used for training. \cosimo{check experiment of kinect to see how to derive it}

==> implementation.tex <==
% !TEX root = egpaper_for_review.tex
\section{Implementation Details}

In this section, we describe the implementation details of learning depth-image embedding. We first discuss how we generate the training data and  the architecture of our network and then describe how we generate training data.

%\subsection{Network Training}
% \begin{figure*}[t!]
%\centering
%\includegraphics[width = \textwidth]{figures/network.pdf}
%\caption{The network structure}
%\label{fig:network}
%\end{figure*}

\

The neural network structure we use for training consists of two main modules: an \emph{extraction} and a \emph{classification} module.
The first module takes a depth image as input and outputs the $d$-dimensional per-pixel feature descriptors. There is a tradeoff in choosing $d$: on the one hand, if $d$ is too small the desciptor cannot discriminate the body segments as the desciptor for distant parts of the body become correlated; on the other hand, using too large a value for $d$ requires many training samples to ensure smoothness. We set $d=16$ which we find to be a good compromise between the two factors.

The simplest architecture for extraction is an AlexNet structure, which is simple and computes a descriptor for each pixel in a depth map independently~(see Table~\ref{table:singlePatch}). This independent \emph{single patch} processing, however, involves redundant computations (since similar pixel neighborhoods are processed repeatedly in different depth image patches) and leads to non-smooth and noisy descriptors, and so is not ideal for our extraction module. We therefore a modification, the \emph{end-to-end structure}, which takes a single depth image as input and computes descriptors for all the pixels simultaneously~(see Table~\ref{table:end-to-end}). In the first layer of the network, we downsample the input image by a factor of 4. This downsampling not only makes the computations faster and more memory efficient, but also removes salt-and-pepper noise which is typical in the output from depth cameras. Second, we modify the pooling and inner product layers to handle whole images~\cite{SermanetEZMFL13}. Finally, we perform upsampling in the last layer by using neighborhood information in a 3-by-3 window. This upsampling implicitly performs linear smoothing between the descriptors of neighboring pixels. It is possible to further smooth the descriptors of neighboring pixels in a post-processing step, but as shown in our results, this is not necessary since our network is capable of extracting smooth and reliable descriptors.

\input{table/patch}
\input{table/whole_image}

\duygu{Peter and cosimo, can you please help to write the remaining text in this section?}
The fully connected layer 2xfc is equivalent to 1x1 convolutional layer, therefore we simply replaced 2xfc with ??. Max pooling layer reduces the height and width of an image by one half, but for our whole image network the output of each pixel needs to be computed from different selection of poolings. Although previous work such as ??? uses only one specific pooling positions and approximate the others, we record the result of all 4 different offsets of pooling layer and compute the next layer based on each of those independently. Therefore, after our modified max pooling layer the height and width of each image reduce by half, and the number of resulting images is 4 times of the number of input images.

\cosimo{bilinear interpolation is one kind of up-sampling convolution, thus our network cannot be worse than that}

After ??? we interleave the pixels from 64 sub layers back to a single layer, resulting in an output of 128 by 128 pixels, with 4096 channels. We can apply the ??? to convert each pixel to be a 16 channel descriptor, and then use bilinear interpolation to get 512 by 512 descriptors. Note that the bilinear interpolation is actually an up-sampling convolution, whose kernel is of size 3 by 3 (!!! need figure). Here we apply relaxation to allow learnable weights of the up sampling. Furthermore, we merge the two layers together, without inserting activation layer in between. Therefore it's equivalent to learning a convolutional kernel of size 3x3x4096, and output size 4x4x16.



\cosimo{for the second part we also replace inner product layers by 1x1 convolutional layers.
And loss function is defined by the sum of loss of every pixel.}

\mypara{Classification} The second module, the classification module, receives the per-pixel descriptors and labels each pixel with one of the possible segment classification labels. Specifically, this module first computes the dot product of the input feature descriptor vector with each of the $N$ representative descriptors for the possible labels. Then a \emph{softmax} layer converts the computed dot products into probabilities of the input descriptor belonging to each of the possible labels. The predicted label for the input descriptor is the label with the highest probability. This prediction is compared with the ground truth label using multinomial logistic regression and the loss of all input descriptors are accumulated to generate a single loss value for the classification module. Since we adopt an overlapping smoothing strategy using multiple segmentations of the human template, each pixel in a depth image might belong to different segments on different segmentations. We therefore connect the extraction module to multiple classification modules, one per segmentation. The final loss output of the network is computed by simply averaging the loss values of all the classification modules.


\subsection{Training Data Collection}
To train our network, we collected 3D models from various data sets. For each 3D model, we rendered depth maps from various camera viewpoints to feed as input to our network. We used a depth image size of $512 \times 512$ pixels, where the rendered human character covers roughly half of the height of the depth image. This setup is comparable to the data provided by commercial depth cameras; for example, the Kinect $v.1$ camera provides a depth map with resolution $512 \times 424$, where a human of height $1.7$ meters standing $2.5$ meters away from the camera has a height around $288$ pixels in the depth image.
% FOV = 53.8 degrees
% height = 2*tan(53.8/2)*2.5 = 2.537
% 1.7/2.5*424 = 288.32

For every depth image, we assume that the background can be discarded easily (both during training and testing). For data generated by rendering 3D models, this is a trivial matter of zero-filling the background; for data acquired from commercial depth sensors, we segment the background either by discarding pixels whose depth exceeds a certain threshold, or pre-record the background and subtract it during capture. %In our experiments, we find these two criteria to be sufficient for captures acquired in indoor environments.

%Once the background is segmented out from a depth image, we compute the mean depth value for the foreground pixels and subtract it from each recorded depth value to produce a zero-mean depth image. Please note that, we do not normalize the depth values by dividing by a value computed per frame because this would lead to inconsistent depth ranges across different depth images of humans in different poses and rendered from different viewpoints. However, when using a new depth camera with a different unit of depth measurement, a constant scaling should be applied to have a consistent depth range as the training data.
%
We now describe the 3D data sets we have used for generating training data. The data sets used for evaluating our algorithm will be discussed in Section~\ref{sec:results}.

\mypara{SCAPE dataset} One of the main sources of training data for our system is the SCAPE database~\cite{Anguelov:2005} which provides $71$ registered meshes of a person in different poses. We consistently segmented each of these registered meshes into $500$ regions in order to generate classification labels. We rendered each of these segmented meshes from $144$ different viewpoints to generate training depth images. As explained in Section~\ref{sec:smoothing}, in order to eliminate artifacts due to segmentation boundaries, we performed $5$ different segmentations. Since the SCAPE database provides ground truth dense correspondences between any pair of meshes, we computed these segmentations only once, and transfer them to all the meshes.

\mypara{MIT dataset} We used all the animation sequences provided by Vlasic et al.~\cite{Vlasic:2008:AMA} except the \emph{samba} and \emph{swing} sequences, which we reserve for evaluation. As for the SCAPE database, for each sequence we compute $5$ different segmentations of $500$ regions each. We rendered each animation sequence to depth images from 36 different viewpoints. To establish correspondences across different animation sequences, we manually annotated 33 semantic landmark points (e.g. left shoulder, right shoulder, left hip, right hip etc.) on a representative 3D mesh from each data set, then propagated these annotations to the rest of the sequences. We fed the annotated landmark points across all the animation sequences as additional training data to our network.

\mypara{Yobi3D dataset} We downloaded $2000$ human models from the Yobi3D data set~\cite{Yobi3D}, which includes models in different poses and with different clothing. Even though this data set provides rich variation in clothing, it does not contain any ground truth correspondence between models. Therefore we consistently annotated $33$ semantic landmark points on each 3D model by hand (annotation data is available in the supplementary material) and rendered $144$ depth images from different viewpoints. We used the annotations as training data for our network.

For depth images that are provided by segmentation, every foreground pixel's classification error on all segmentation region it belongs to is accumulated in the objective function. And for depth images generated for annotating classification, only pixels closed to the annotated vertices are used as only pixels near our landmarks are semantically consistent.


==> overview.tex <==
% !TEX root = egpaper_for_review.tex
\begin{figure*}[t]
\begin{center}
   \includegraphics[width=\textwidth]{figures/pipeline/pipeline.pdf}
\end{center}
   \caption{We train a neural network which extracts a feature descriptor and predicts the corresponding segmentation label on the human body surface for each point in the input depth maps. We generate per-vertex descriptors for 3D models by averaging the feature descriptors in their rendered depth maps. We utilize the extracted features to compute dense correspondences.}
\label{fig:pipeline}
\end{figure*}

\section{Problem Statement and Overview}
We introduce a deep learning framework to compute dense correspondences across full or partial human shapes. We train our system using depth maps of humans which can also be utilized to establish correspondences between full and partial scans.
 
Given depth maps of two humans $I_1$, $I_2$, our goal is to determine which two regions $R_i\subset I_i$ of the depth maps come from corresponding parts of the body, and to find the correspondence map $\phi: R_1\to R_2$ between them. Our strategy for doing so is to formulate the correspondence problem first as a \emph{classification} problem: we learn a feature descriptor $\mathbf{f}: I \rightarrow R^d$ which maps each pixel in a \emph{single} depth image to a feature vector. We then utilize these feature descriptors to establish correspondences across depth maps~(see Figure~\ref{fig:pipeline}). We desire the feature vector to satisfy two properties:
\begin{enumerate}
\item $\mathbf{f}$ depends only on the pixel's location on the human body, so that if two pixels are sampled from the same anatomic location on depth scans of two different humans, their feature vector should be nearly identical, irrespective of pose, clothing, body shape, and angle from which the depth image was captured;
\item $\|\mathbf{f}(p)-\mathbf{f}(q)\|$ is small when $p$ and $q$ represent nearby points on the human body, and large for distant points on the body.
\end{enumerate}
To formalize these properties, we first choose a canonical \emph{human body template} $T$, a surface in $\mathbb{R}^3$ in the shape of an \emph{average} human. Distance between points on the human body can be expressed as geodesic distance on $T$. Formally, the above two propreties are then the requirement that if two pixels $x_1$ and $x_2$ on depth maps correspond to 3D points $p(x_1)$ and $p(x_2)$ on $T$, the function $f$ satisfies
\begin{eqnarray}
D(p(x_1), p(x_2)) < \varepsilon_1 \Rightarrow \|f(x_1) - f(x_2)\| < \delta_1 \label{eqn:constraint1}\\
D(p(x_1), p(x_2)) > \varepsilon_2 \Rightarrow \|f(x_1) - f(x_2)\| > \delta_2 \label{eqn:constraint2}
\end{eqnarray} 
for tolerances $\varepsilon_i, \delta_i$.

A possible approach to train a network to learn such a mapping with these properties is to sample pairs or triplets of points on the training images, and directly enforce these properties using siamese or triplet-loss energies. However, this approach requires a dense sampling strategy, which is computationally expensive. In addition, choosing the right sampling strategy for the pairs/triplets is often a non-trivial task~\cite{SchroffKP15}. Instead, we draw inspiration from data-driven 2D image correspondence methods, where deep neural networks trained to perform classification tasks have been commonly used to extract feature descriptors. 

\subsection{Embedding Learning as a Classification Task}
%We now describe in detail how we can learn a feature descriptor that satisfies the desired constraints given in Equation~\ref{eqn:constraint1} and~\ref{eqn:constraint2}.
Traditional classification networks, such as AlexNet~\cite{NIPS2012_4824}, predict the classification label of an input $x$ by first extracting a feature descriptor $f(x)$ and feeding this into the last layer of the network, which uses a set of linear predictor functions to perform the actual classification. This last step can be interpreted as multiplication of the feature vector by a matrix $M_{N \times d}$, where $d$ is the dimension of $f(x)$, $N$ is the number of classification labels, and each row of $M$ can be regarded as a representative descriptor $\beta_i$ for the corresponding class label. The label for $x$ is selected using
\begin{equation}
y = \argmax_i{\langle f(x), \beta_i\rangle}.
\end{equation}
%Since scaling $f(x)$ leaves the relative magnitudes of these inner products unchanged, we can assume $f(x)$ is normalized, $\|f(x)\| = 1$. Similarly, we can assume each class representative descriptor is also unit length, $\| \beta_i \| = 1$. 
% this is wrong:
%
%Then, $\langle f(x), \beta_i\rangle = 1 - \|f(x) - \beta_i\|_2^2/2$ becomes a monotonically decreasing function of the Euclidean distance between  $\beta_i$ and $f(x)$. Therefore, finding the maximum value of $f(x)^T\beta_i$ is equivalent to finding the $f(x)$ that is closest to $\beta_i$.

The goal of the classification network is thus to learn \emph{both} the descriptor $f(x)$ and the representative descriptors $\beta_i$ for each of the class labels. This process tends to learn well-separated $\beta_i$, so that an input belonging to a certain class will produce a large dot product only with the corresponding $\beta_i$. In addition, the network tends to pull the descriptors of the input points closer to the representative descriptors of their corresponding labels to maximize their dot product. Consequently, if two points $x_i$ and $x_j$ belong to two different classes $i$ and $j$, typically $\|f(x_i) - f(x_j)\|$ is large, and two points belonging to the same class will tyically be mapped to nearby points in the feature space. Our approach is to benefit from this property of classification networks by segmenting the human template model $T$ into regions, where points in the same region are geodesically close. We then formulate a classification learning task as described above, where the input $x$ are a depth map and a pixel of interest, and the classification labels are the segmented regions; the resulting descriptor will then map points corresponding to nearby regions on the body to nearby points in feature space.

\subsection{Learning a Smooth Embedding}
\label{sec:smoothing}
\begin{figure}[t]
\begin{center}
   \includegraphics[width=1.0\linewidth]{figures/segmentation/segmentation.pdf}
\end{center}
   \caption{Segmentation.}
\label{fig:segmentation}
\end{figure}

As explained, embedding learning can be formulated as a classification task by segmenting the human body into regions and predicting the region label for each input. A potential drawback of this approach is that nearby points straddling a region boundary do not necessarily have nearby feature descriptors: for any pair of pixels corresponding to 3D points close to each other on the human body, but classified into different regions by the segmentation, the classification network would learn non-smooth feature descriptors that are far apart from each other by pulling each pixel's feature vector closer to its region's representative descriptor. In order to eliminate such artifacts, we propose to compute \emph{multiple} segmentations of $T$, with different segment boundaries, to increase the chance that a pair of nearby points belong to the same region in at least one segmentation. 

In order to build a sufficiently large set of segmentations, we first generate many candidate segmentations ($100$ in our experiments) with $k$ regions each ($k=500$ in our experiments). Each segmentation is generated by randomly sampling $k$ vertices on the human model via a farthest point sampling strategy, and constructing the corresponding Voronoi diagram. We then pick one of these segmentations randomly to be a part of our final segmentation set. At each iteration, we pick a new segmentation whose intersection with all of the previously-selected segmentations produces the maximum number of regions on the human body. We stop selecting new segmentations when the increase in the number of generated regions by intersection slows down. In our experiments we find out that a segmentation set of $5-10$ segmentations is sufficient. %\etienne{I'm confused by this procedure. Why does the number of new regions ever decrease? What does "increase significantly" mean?}

Given this set of multiple segmentations, where the label of a particular pixel may vary across different segmentations, the goal of the network is then to learn a feature descriptor for depth map pixels, and representative descriptors for each region on each segmentation, so that each pixel is correctly classified on as many segmentations as possible.

\subsection{Correspondence Computation}
Our trained network can be utilized to extract per-pixel feature descriptors for depth maps. We use these descriptors to establish correspondences simply by a nearest neighbor search in the feature space~(see Figure~\ref{fig:pipeline}). We further extend our method to establish correspondences between full/partial 3D scans. We first render depth maps of each 3D scan from various multiple viewpoints and compute per-pixel descriptors for each of these depth images. A per-vertex feature descriptor is then computed by averaging the descriptors of the pixels it projects to in each depth map it is visible in.
%Since depth images only provide partial observations of the human body, the correspondence computation should consider the fact that the overlapping regions between two depth images is often smaller than the regions observed by each of the depth images alone. Thus, we need a strategy to discard unreliable correspondences coming from non-overlapping regions. We achieve this goal by enforcing spatial constraints among the correspondences since neighboring pixels in a source depth image are likely to be matched to neighboring pixels in the target depth image. More specifically, we build a connection graph in the source depth image where each pixel is denoted by a vertex. Two neighboring pixels $p^s_1$ and $p^s_2$ in the source depth image (we only consider horizontal or vertical neighbors) are connected by an edge if their corresponding pixels $p^t_1$ and $p^t_2$ in the target image represent 3D points with a Euclidean distance below a certain threshold ($10$ centimeters in our example). We then extract the largest connected component of this graph and discard the remaining correspondences.



